Predicting tacrolimus exposure in kidney transplanted patients using machine learning

Tacrolimus is one of the cornerstone immunosuppressive drugs in most transplantation centers worldwide following solid organ transplantation. Therapeutic drug monitoring of tacrolimus is necessary in order to avoid rejection of the transplanted organ or severe side effects. However, finding the right dose for a given patient is challenging, even for experienced clinicians. Consequently, a tool that can accurately estimate the drug exposure for individual dose adaptions would be of high clinical value. In this work, we propose a new technique using machine learning to estimate the tacrolimus exposure in kidney transplant recipients. Our models achieve predictive errors that are at the same level as an established population pharmacokinetic model, but are faster to develop and require less knowledge about the pharmacokinetic properties of the drug.

==> old_tables/experiments1.tex <==
\begin{table}
%   \scriptsize
    %\normal
    \caption{\label{tab:experiments1}Results from the experiments on predicting the area under the concentration versus time curve.
    }
    \centering
   \begin{tabular}{p{0.15\textwidth}p{0.05\textwidth}
    p{0.1\textwidth}p{0.1\textwidth}} 
    \toprule 
         Model number & Fixed time points & Flexible time points approach $1$ & Flexible time points approach $2$  \\
         \midrule
         \% relative RMSE on test set* \\
         \midrule
         $1$ & $9.39$ & $15.06$ & $14.60$ \\
         $2$ & $14.47$ & $15.24$ & $9.94$ \\
         $3$ & $4.94$ & $6.44$ & $8.65$\\
         $4$ & $11.82$ & $9.37$ & $8.47$ \\
         $5$ & $11.90$ & $26.08$ & $19.18$ \\
         \midrule
         Mean & $10.50$ & $14.44$ & $12.17$ \\
         \bottomrule
         \multicolumn{4}{p{0.7\linewidth}}{Abbreviations: RMSE = root mean squared error. The first approach is when the concentration and the time deviation is provided directly to the model. The second approach is when the concentration at 3 hours is estimated based on the two last concentrations. * \% relative root mean squared error is calculated by dividing the root mean squared error by the mean target value of the test set. } \\
    \end{tabular}
\end{table}

==> old_tables/experiments_simulated1.tex <==
\begin{table}
%   \scriptsize
    %\normal
    \caption{\label{tab:experiments_sim1}Results for the first modeling approach for flexible time points when increasing numbers of simulated patients are included in the training data set. The test data sets remain the same as in earlier experiments.
    }
    \centering
   \begin{tabular}{p{0.1\textwidth}p{0.05\textwidth}
    p{0.075\textwidth}p{0.075\textwidth}p{0.075\textwidth}} 
    \toprule 
         Model number & Real patients & Real patients and $2.000$ simulated patients & Real patients and $6.000$ simulated patients & Real patients and $50.000$ simulated patients  \\
         \midrule
         \% relative RMSE on test set* \\
         \midrule
         $1$ & $15.06$ & $10.01$ & $8.74$ & $8.72$ \\
         $2$ &  $15.24$ & $12.23$ & $12.54$ & $11.49$ \\
         $3$ &  $6.44$ & $4.24$ & $4.62$ & $5.23$\\
         $4$ &  $9.37$ & $9.62$ & $9.70$ & $8.71$\\
         $5$ &  $26.08$ & $7.25$ & $7.26$ & $7.58$ \\
         \midrule
         Mean & $14.44$ & $8.67$ & $8.57$ & $8.35$\\
         \bottomrule
         \multicolumn{4}{p{0.7\linewidth}}{Abbreviations: RMSE = root mean squared error. * \% relative root mean squared error is calculated by dividing the root mean squared error by the mean target value of the test set. } \\
    \end{tabular}
\end{table}

==> old_tables/experiments_simulated2.tex <==
\begin{table}
%   \scriptsize
    %\normal
    \caption{\label{tab:experiments_sim2}Results for the second modeling approach for flexible time points when increasing numbers of simulated patients are included in the training data set. The test data sets remain the same as in earlier experiments.
    }
    \centering
   \begin{tabular}{p{0.1\textwidth}p{0.05\textwidth}
    p{0.075\textwidth}p{0.075\textwidth}p{0.075\textwidth}} 
    \toprule 
         Model number & Real patients & Real patients and $2.000$ simulated patients & Real patients and $6.000$ simulated patients & Real patients and $50.000$ simulated patients  \\
         \midrule
         \% relative RMSE on test set* \\
         \midrule
         $1$ & $14.60$ & $13.30$ & $9.68$ & $12.33$ \\
         $2$ &  $9.94$ & $14.67$ & $14.19$ & $14.44$ \\
         $3$ &  $8.65$ & $7.68$ & $9.39$ & $7.81$\\
         $4$ &  $8.47$ & $12.76$ & $11.43$ & $12.17$\\
         $5$ &  $19.18$ & $16.02$ & $15.27$ & $18.12$ \\
         \midrule
         Mean & $12.17$ & $12.89$ & $11.99$ & $12.97$\\
         \bottomrule
         \multicolumn{4}{p{0.7\linewidth}}{Abbreviations: RMSE = root mean squared error. * \% relative root mean squared error is calculated by dividing the root mean squared error by the mean target value of the test set. } \\
    \end{tabular}
\end{table}

==> old_tables/leave_one_out.tex <==
\begin{table}
%   \scriptsize
    %\normal
    \caption{\label{tab:loo_1}Results from leave one out cross validation on the first visit for the $68$ patients. A dummy regressor that always predicts the mean target value was used as a baseline model for comparison. 
    }
    \centering
   \begin{tabular}{p{0.1\textwidth}p{0.07\textwidth}
    p{0.07\textwidth}p{0.07\textwidth}p{0.07\textwidth}} 
    \toprule 
         \% relative RMSE* & All time points & $3$ fixed time points & $3$ fixed time points, less features & Baseline model \\
         \midrule
          &$9.46$ & $10.72$ & $11.18$ & $29.23$ \\
         \bottomrule
         \multicolumn{4}{p{0.7\linewidth}}{Abbreviations: RMSE = root mean squared error. The $3$ fixed time points included concentrations measured at $0$, $1$ and $3$ hours after drug administration. * \% relative root mean squared error is calculated by dividing the root mean squared error by the mean target value of the training data set. } \\
    \end{tabular}
\end{table}

==> old_tables/leave_one_patient_out.tex <==
\begin{table}
%   \scriptsize
    %\normal
    \caption{\label{tab:leave_patient_out1}Results from leave one patient out cross validation on the first visit for the $68$ patients. The results are reported as \% relative RMSE.
    }
    \centering
   \begin{tabular}{p{0.15\textwidth}p{0.05\textwidth}
    p{0.1\textwidth}p{0.1\textwidth}} 
    \toprule 
         First approach \\
         \midrule
         Feature for time difference & Features for absolute time & Combination of two first & Combination of two first, more features\\
         \midrule
         $15.99$ & $18.21$ & $16.43$ & $15.37$ \\
         \midrule
         Second approach \\
         \midrule
         Linear regression & `Reverse' linear regression & Log-linear regression & Population PK model\\
         \midrule
         $17.04$ & $18.40$ & $16.09$ & $14.89$ \\
         \bottomrule
         \multicolumn{4}{p{0.7\linewidth}}{Abbreviations: RMSE = root mean squared error. PK = pharmacokinetic. * \% relative root mean squared error is calculated by dividing the root mean squared error by the mean target value of the training data set. } \\
    \end{tabular}
\end{table}

==> removed_parts.tex <==

%Our models achieve predictive errors that are at the same level as an established population pharmacokinetic model,...


%Using only the two closest concentrations might give more accurate estimations, considering that a 2-compartment model best describe tacrolimus pharmacokientics, and should be tested as future work.

%To increase applicability in the clinic, we focus on trough concentrations and concentrations measured within the first three hours after drug administration, i.e. one and three hours.

%\section{Related work}
  
%Related work not ML for AUC predictions:
%Other studies have developed \ac{ML} models to directly predict personalised tacrolimus doses in renal transplanted patients~\cite{tang2017TacDose,fu2021machine}. Despite their clinical relevance, these models can not be used for predicting the effect of a given dose.

% ---------------------------------------------
%\subsection{Renal transplantation and tacrolimus}
% ---------------------------------------------
%Kidney transplantation is the preferred option of treatment during terminal kidney failure~\cite{abecassis2008kidneyTx}. Following organ transplantation, the patient needs life-long immunosuppression in order to prevent rejection of the transplanted organ. Tacrolimus is a part of the standard immunosuppressive treatment protocol after renal transplantation in most centers around the world~\cite{brunet2019consensus}. Unfortunately, it is challenging to find the optimal dose for a new patient due to the high variation in drug exposure between individuals and also within the same individual over time. Too low exposures of tacrolimus might lead to rejection of the new organ, while too high exposures will increase the risk of experiencing severe side effects such as diabetes, infections, hypertension and impaired renal function~\cite{mayer1997adverse,liverGroup1994adverse}. Consequently, therapeutic drug monitoring, where the clinician decides the dose based on whole blood drug concentrations, is necessary in order to obtain an appropriate drug regimen~\cite{brunet2019consensus}. 

%In order to estimate the tacrolimus exposure, the clinicians can either examine the trough concentration or the \ac{AUC}. An illustration of a drug concentration versus time curve is provided in~\cref{fig:example_auc}. The \ac{AUC} is recognized as more accurate in order to reflect the drug exposure. Unfortunately, it requires a lot of resources and is less convenient since the patient needs to be available for blood sampling during the whole dose interval. For tacrolimus, this interval is $12$ hours when the drug is administered twice daily. Consequently, the trough concentration is most commonly used, even though it is regarded as less optimal. To make the \ac{AUC} more applicable, a method that can accurately estimate the \ac{AUC} value for an individual patient would be needed. 

%\begin{figure}[!tb]
    %\centering
    %\includegraphics[width=0.5\textwidth]{figures/Tac_exampleAUC.pdf}
    %\caption{\label{fig:example_auc}
    %A drug concentration versus time curve. The area under the curve represents the systemic drug exposure. Crosses represent the measured drug concentrations.
    %}
%\end{figure}


%First, a feature representing the difference in time between the desired time at three hours and the actual time point were included. The second combination did instead include the exact time points for all three concentrations measured in minutes after transplantation. Next, the features from the two first combinations were combined together with patient characteristics (body weight and height, sex, body mass index, body surface area, hematocrit and type of assay for the analysis). Finally, the two first combinations were combined without adding extra patient characteristics.

%For the second approach, several methods for estimating the concentration after three hours were explored. First, linear regression using the concentrations measured at one hour and the latest time point was applied to estimate the concentration at three hours. Also, a version was implemented were the one hour concentration and last concentration were swapped if the last concentration was higher than the concentration measured at one hour. This was done in order to prevent the estimated concentration at three hours to become unrealistically high, as the maximum concentration most likely arise before three hours. The approach is referred to as `reverse linear regression' in the following sections. Third, log-linear regression between the latest concentration and the trough concentration were applied for prediction of the three hours concentration. Finally, an earlier developed population \ac{PK} model~\cite{aasberg2013popPKmodel} estimated the concentration at three hours based on patient characteristics, the measured trough concentration as well as the concentrations measured at one hour and the last time point.


%Removed from the discussion section: 
%First, the estimation of missing drug concentrations will introduce some uncertainty because they can deviate from the true, unknown concentrations. The estimations will be less accurate when the number of available concentrations is small. If the estimated concentrations deviate a lot from the unknown, true values, it can make it difficult for the models to make accurate \ac{AUC} estimations. This will especially affect the results from the experiments that include all sixteen time points and the flexible time points, since more concentrations were estimated in these datasets.


%Removed from the introduction: 
%Criticism of ML: they are not transparent and we cannot understand the pharmacokinetic processes from the model. However, with the use of explainable AI, it is possible to identify which features (i.e., patient characteristics) that are most important for the model. 

==> tables/leave_one_patient_out.tex <==

\begin{table}
%   \scriptsize
    %\normal
    \caption{\label{tab:leave_patient_out1}Results from model development where the time point for measuring the last drug concentration was allowed to deviate, see main text for details. Leave one patient out cross validation was applied for the first visit for the $68$ patients.
    }
    \centering
   \begin{tabular}{p{0.3\textwidth}p{0.07\textwidth}} 
    \toprule 
          & \% relative RMSE* \\
         \midrule
         \textbf{First approach} \\
         Feature for time difference & $16.88$\\ 
         Features for exact time & $17.36$\\ 
         Combination of two first & $16.65$\\ 
         Combination of two first, more features & $15.98$\\
         \midrule
         \textbf{Second approach} \\
         Linear regression & $17.20$ \\ 
         `Reverse' linear regression & $18.15$ \\
         Log-linear regression & $16.25$\\
         Population PK model concentration & $16.27$\\
         \bottomrule
         \multicolumn{2}{p{0.92\linewidth}}{Abbreviations: RMSE = root mean squared error. PK = pharmacokinetic. * \% relative root mean squared error is calculated by dividing the root mean squared error by the mean target value of the training data set. } \\
    \end{tabular}
\end{table}
